Towards a Symbolic-Numeric Method to Compute Puiseux Series: The Modular Part

We have designed a new symbolic-numeric strategy to compute efficiently and accurately floating point Puiseux series defined by a bivariate polynomial over an algebraic number field. In essence, computations modulo a well chosen prime $p$ are used to obtain the exact information required to guide floating point computations. In this paper, we detail the symbolic part of our algorithm: First of all, we study modular reduction of Puiseux series and give a good reduction criterion to ensure that the information required by the numerical part is preserved. To establish our results, we introduce a simple modification of classical Newton polygons, that we call "generic Newton polygons", which happen to be very convenient. Then, we estimate the arithmetic complexity of computing Puiseux series over finite fields and improve known bounds. Finally, we give bit-complexity bounds for deterministic and randomized versions of the symbolic part. The details of the numerical part will be described in a forthcoming paper.

==> conclusion.tex <==
\section{Conclusion}

This paper summarizes the results we have obtained regarding the
symbolic part of our program towards a fast and reliable method
to compute Puiseux series with floating point coefficients.
In particular, the criterion ensuring preservation of polygon trees is
essential. %Details are in \cite{poteaux-rybowicz08}.

Along the path, we have derived improved complexity bounds for
the computation of Puiseux series over finite fields. 
Although not optimal, these bounds are quite reasonable, i.e.
quadratic in the output size, up to a factor $d$.
%These results for Puiseux series above 0 can easily be extended to 
%show that Puiseux series above {\em all} critical points can
%be computed within the same $\Ot$ asymptotic cost.
Refinements may be obtained by optimizing 
several steps of our complexity analysis. It is not clear
that these refinements may significantly improve the
final asymptotic cost.

Bit-complexity estimates
for the Monte-Carlo version of the first stage of our symbolic-numeric
method confirm that the coefficient growth of pure symbolic Newton-Puiseux
algorithm is avoided. Complexity bounds for the Las Vegas
and deterministic versions can be obtained similarly.
An analogous bit-complexity bound can also be
deduced for the computation of the genus of an algebraic curve
defined over an algebraic number field.

The numerical part of the algorithm is still being investigated
and several variants are being compared.

The scope of our symbolic-numeric strategy may be broader~: 
For instance, series solutions at singular
points of certain linear differential equations can be constructed using
Newton polygons. It would be interesting to investigate the benefits 
of our approach in this context.


==> myopt.tex <==
\usepackage{graphicx}

\let \dd = \displaystyle
\let \bs = \backslash
\let \E = \exists
\let \V = \forall
 
